Multi-Type Activity Recognition in Robot-Centric Scenarios

Activity recognition is very useful in scenarios where robots interact with, monitor or assist humans. In the past years many types of activities -- single actions, two persons interactions or ego-centric activities, to name a few -- have been analyzed. Whereas traditional methods treat such types of activities separately, an autonomous robot should be able to detect and recognize multiple types of activities to effectively fulfill its tasks. We propose a method that is intrinsically able to detect and recognize activities of different types that happen in sequence or concurrently. We present a new unified descriptor, called Relation History Image (RHI), which can be extracted from all the activity types we are interested in. We then formulate an optimization procedure to detect and recognize activities of different types. We apply our approach to a new dataset recorded from a robot-centric perspective and systematically evaluate its quality compared to multiple baselines. Finally, we show the efficacy of the RHI descriptor on publicly available datasets performing extensive comparisons.

==> introduction.tex <==
% Drop letter for first word of the Introduction 
% Here we have the typical use of a "T" for an initial drop letter
% and "HIS" in caps to complete the first word.
\IEEEPARstart{T}{he} recognition of activities is a crucial problem in computer vision. % Use only for final RAL version
Usually, activities are categorized based on how many people participate (one person, two persons, a group of people), and the point of view from which they are recorded (third person, ego-centric). The combination of these two characteristics generates $6$ possible \textit{types} of activities. Traditional computer vision methods address the recognition of only one \textit{type} of activity. For example, single person activities from a third-person perspective \cite{laptev03} has been studied broadly in the past. Two-person interactions from a third person perspective \cite{ryoo09} and group activities from a third point of view \cite{khamis12} have been analyzed more recently. In the last few years, the ego-centric perspective has been largely explored in the form of ego-centric activities \cite{grauman13,fathi11}, where the goal is understanding what the person wearing the camera is doing, and ego-centric interactions \cite{ryoo13,lu15}, where a robot usually wears a camera, and the objective is classifying what activities other people are doing to the robot.

In all the above-mentioned cases, videos to be classified belong to a specific \textit{type} of activities. However, imagine a service robot, who provides directions and recommendations in public places, or a robot assistant, who helps elderly people, or yet a surveillance robot, who monitors crowded areas. In these situations, people usually perform several different types of activities at the same time, and the robot should be able to classify them all. For example, it should be able to understand if a person intends to talk to it (ego-centric interactions), to detect if someone needs help (single person activities from a third person perspective), or notify someone if there is a fight (two-persons interactions from a third person perspective). In summary, there is a clear need to move towards a more general objective: classifying more complex scenes where multiple people perform activities of different types concurrently or in a sequence. To our knowledge, ours is the first recognition work that considers such multiple types of activities. We provide a new video dataset recorded from a robot-perspective where multiple activities and interactions happen at the same time, and present a novel approach to appropriately analyze such videos.

\begin{figure*}
\begin{center}
\includegraphics[width=0.85 \textwidth]{RHI_extr_small.png}
\end{center}
\caption{This picture represents how RHIs on skeleton and depth are extracted from a single person (e.g., person1) and pairs of persons (e.g., $\{$person1, person3$\}$ and $\{$person2, person3$\}$). For RHIs on skeletons, the relations between pairs of joints are computed for each frame, for each pair. For RHIs on depth, the Hamming distance between strings obtained from the $\tau$ test represents the relations between local regions. The first descriptor in a temporal window is subtracted to each other frame in the window; these differences are then convoluted with a set of Gaussian filters. The filter responses are summed to generate the final RHI descriptor over the window of frames.}
\label{fig:rhiextr}
\end{figure*}
In order to discriminate different types of activities, a \textit{unified} descriptor, i.e., a descriptor that can be extracted from several activity types, is necessary. We propose a new \textit{unified} mid-level descriptor, called \textit{Relation History Image} (RHI) (see Fig. \ref{fig:rhiextr}). The Relation History Image is built as the variation over time of relational information between every pair of local regions (joints or image patches) belonging to one or a pair of subjects. It can be extracted from several types of activities while maintaining the same format and dimensionality, thereby allowing the direct comparison between activity videos of completely different types. This direct comparison enables the robot to detect ongoing activities and discard false positives even in the scenario where multiple types of activities are present in the same video. In contrast to the other previous appearance-based unified descriptors such as STIP \cite{laptev03} or DSTIP \cite{lu13}, RHI is suitable to represent subtle interactions where human body configurations are very important. The presented experiments confirm that RHI significantly outperforms state-of-the-art descriptors in our scenario, as well as on other public datasets.

% thus it is possible to directly compare (i.e., classify) activities of completely different types. 

% This allows us to train multiple types of activities with the same classifier and obtain comparable results for such activities when they are present in the same scene, sequentially or concurrently. In order to recognize all ongoing activities while discarding false positives, we need comparable classification scores between interactions, single person activities and ego-centric interactions,

%The main peculiarity of multi-type activity videos is that it is impossible to know a priori who is performing a certain type of activity.

The main peculiarity of multi-type activity videos is that it is impossible to know a priori who is performing what types of activities. In traditional videos with single person actions, it is assumed that each person is doing something singularly. In traditional videos of two-person interactions, it is expected that there are two persons and that they are interacting. In our case, if there are three persons in the scene, there is no way of knowing a priori if two of those persons are interacting and who they are, or if some of them are interacting with the robot, or if all three of them are on their own. To solve this problem, we propose a new method based on optimization. First, RHI descriptors are extracted from all the possible combinations of subjects in the scene, including those formed by pairing each subject with himself. All the combinations are fed to a classifier, which provides for each descriptor the confidence that it belongs to a certain class. Since RHI can be extracted from different types of activities, the resultant class can be an interaction, or an action, or an interaction with the robot. An optimization problem based on the generated confidence returns who is performing a certain type of activity, and what activity that is. In the example above, a possible outcome of our algorithm is: \textit{person1-person3 hug, person2 sit}. Notably, the optimization problem outputs both the action and who is involved in it.

Our main contribution is the idea of recognizing concurrent activities belonging to different \textit{types}, which is crucial in real-world scenarios. Our technical contributions are: 1) a new \textit{unified} descriptor, RHI, which can be extracted from multiple types of activities and thus simplifies the classification step; 2) a new method to identify what persons are involved in what activity; 3) a systematic evaluation to compare the proposed approach to several baselines on a newly collected dataset as well as on public ones.

